Convex Optimization-Based Model Predictive Control for the Guidance of Active Debris Removal Transfers

Active debris removal (ADR) missions have garnered significant interest as means of mitigating collision risks in space. This work proposes a convex optimization-based model predictive control (MPC) approach to provide guidance for such missions. While convex optimization can obtain optimal solutions in polynomial time, it relies on the successive convexification of nonconvex dynamics, leading to inaccuracies. Here, the need for successive convexification is eliminated by using near-linear Generalized Equinoctial Orbital Elements (GEqOE) and by updating the reference trajectory through a new split-Edelbaum approach. The solution accuracy is then measured relative to a high-fidelity dynamics model, showing that the MPC-convex method can generate accurate solutions without iterations.

==> Resultsoption1.tex <==
\subsection{Determination of $DC'$}
Before running the guidance scheme, it is ideal to establish an adequate duty cycle value to calculate the reference. If $DC'$ is too small, the reference trajectory would be highly time-consuming, leading to many MPC segments and a high accumulation of thrust errors that result in many recomputations. If $DC'$ is high/close to $DC$, no thrust margin is present to be used to resolve minor deviations from the PMDT trajectory, again leading to recomputations. As recalculating the PMDT solution mid-trajectory results in additions to the time of flight and the fuel consumption, it is reasonable to attempt to limit the number of recomputations required.  

\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.8\textwidth]{Figures/DCplot.jpg}
    \caption{$DC'$ vs time of flight and $\Delta v$}
    \label{DCplot}
\end{figure}

Figure \ref{DCplot} illustrates the variation of real and reference time of flights and $\Delta v$ with the reference duty cycle value. Note that the actual results are obtained assuming no thrust errors.  It can be seen that at $DC' \approx 0.45$ the real and reference values have the most agreement and requires the least number of recomputations.

\subsection{Time optimal results}

Figures \ref{topt12}, \ref{topt22} and \ref{topt32} illustrates the time optimal results obtained. The initial reference is a trajectory of $\Delta v = 161.34$ m/s and $TOF = 55.70$ days. The actual trajectory (following two recomputations) requires $\Delta v = 161.095$ m/s and $TOF =   53.66752$ days. At the end of the trajectory, the error in semi major axis, inclination and RAAN are 0.225 km,  0.000081 deg and 0.00492 deg, respectively. 


\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.8\textwidth]{Figures/topt12.png}
    \caption{The time optimal solution with the PMDT recomputations }
    \label{topt12}
\end{figure}
\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.8\textwidth]{Figures/topt22.png}
    \caption{$\Delta v'$ vs time of flight}
    \label{topt22}
\end{figure}
\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.8\textwidth]{Figures/topt32.png}
    \caption{The evolution of semi major axis, inclination and RAAN errors with respect to the reference trajectories}
    \label{topt32}
\end{figure}




\subsection{Fuel optimal results}



Figures \ref{fopt12}, \ref{fopt22} and \ref{fopt32} illustrates the fuel optimal results obtained. The initial reference is a trajectory of $\Delta v = 147.91$ m/s and $TOF = 66.60 $ days. The actual trajectory (following two recomputations) requires $\Delta v =  148.096$ m/s and $TOF =   64.42$ days. At the end of the trajectory, the error in semi-major axis, inclination, and RAAN are 0.028025 km, 0.000064 deg, and 0.00608 deg, respectively. 



\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.8\textwidth]{Figures/fopt12.png}
    \caption{The fuel optimal solution with the PMDT recomputations }
    \label{fopt12}
\end{figure}
\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.8\textwidth]{Figures/fopt22.png}
    \caption{$\Delta v'$ vs time of flight}
    \label{fopt22}
\end{figure}
\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.8\textwidth]{Figures/fopt32.png}
    \caption{The evolution of semi-major axis, inclination, and RAAN errors with respect to the reference trajectories}
    \label{fopt32}
\end{figure}

==> Resultsoption2.tex <==


% \begin{table}[hbt!]
% \centering
% \begin{tabular}{cccc}
% Spacecraft Propagation & TOF (d) & $\Delta v$ (m/s) & $\Delta v^{'}$ (m/s) \\ \hline 
% \multicolumn{4}{c}{Perfect Thrust}                                                                                                      \\
% Low Fidelity  & 262.159 & 144.2285 & 0.0039075 \\
% High Fidelity   & 262.159 & 140.8204 & 0.0013419 \\ \hdashline
% \multicolumn{4}{c}{Low thrust errors}                                                                                                      \\
% Low Fidelity (avg)  & 262.159 & 144.7774 & 0.0054359 \\
% High Fidelity (avg)  & 262.159 & 141.3518 & 0.00080687 \\
% \hdashline
% \multicolumn{4}{c}{High thrust errors}                                                                                                      \\
%  Low Fidelity (avg)  & 262.159 & 145.3054 & 0.0059401 \\
%  High Fidelity (avg) & 262.159 & 141.8686 & 0.00028516  \\
% \hline 
% \end{tabular}
% \caption{Down leg fuel-optimal results}
% \label{td}
% \end{table}




==> extras.tex <==
 % Within the convex optimization, the nodes were set up to be equidistant in true longitude instead of time. The boundary condition on each of the MPC-convex segments was also set in a novel manner, utilizing the proximity quotient of the Q-law \cite{Petropoulos2005} defined as: 
% \begin{equation}
%     Q=\left(1+W_P P\right) \sum_{\oe} W_{\oe} S_{\oe}\left(\frac{d\left(\oe, \oe_T\right)}{\dot{\oe}_{\mathrm{xx}}}\right)^2, \quad \text { for } \oe=a, e, i, \Omega
%     \label{Qlaw}
% \end{equation}
% where $W_p$, $ W_{\oe}$, $P$,$S_{\oe}$, $d\left(\oe, \oe_T\right)$ and $\dot{\oe}_{x \mathrm{xx}}$ represent the scalar weights, the penalty function for the minimum periapsis radius constraint, scaling functions for each of the orbital elements considered, the distance between the current orbital element ($\oe$) and its targeted value ($\oe_T$) and the maximum orbital rates of change.  \par 
% Firstly, the weights are calculated using nonlinear least squares, such that the "time-to-go" from the PMDT solution matches that from the Q law. Then, an estimate of the "time-to-go" at the end of each of the MPC segment ($T_{go}$)  is obtained as follows, based on the variation of semi-major axis, eccentricity, inclination, and RAAN required to reach the final target.
% \begin{equation}
%     \Delta T_{go}(N) = \sqrt{Q} = \sqrt{\left(1+W_P P\right) \sum_{\oe} W_{\oe} S_{\oe}\left(\frac{d\left(\oe_{(N,T)}, \oe_{T}\right)}{\dot{\oe}_{\mathrm{xx}}}\right)^2}
% \end{equation}
% Note that $\oe_{(N,T)}$ is the value that the orbital element should take at the last nodes of the Nth convex-MPC segment, based on the reference PMDT solution.


% Then the constraint on the final node of each of the convex MPC schemes is set as: 
% \begin{equation}
%    |\Delta t_{go}(N)| \leq \alpha T_{go}(N)
% \end{equation}
% where: 
% \begin{equation}
%     \Delta t_{go}(N) = \sqrt{Q} = \sqrt{\left(1+W_P P\right) \sum_{\oe} W_{\oe} S_{\oe}\left(\frac{d\left(\oe_N, \oe_{(N,T)}\right)}{\dot{\oe}_{\mathrm{xx}}}\right)^2}
% \end{equation}
% Note that $\oe_N$ is the orbital element from the convex solution at the last node of the Nth convex-MPC scheme. At the final MPC scheme, $T_{go} = 0$, $|\Delta t_{go}|$ must equal zero, allowing the convex solution to reach the target state precisely. \par 

% Lastly, once the MPC allows the spacecraft to reach the targeted semi-major axis, inclination, and eccentricity, phasing will be conducted via convex optimization, using the Q-law to obtain a reference trajectory. This is yet to be implemented.


% Active debris removal (ADR) missions have gained significant interest as means of mitigating collision risks in space. Autonomy is crucial to having such missions in large scale, as well as for lowering their operational costs. This work explores the use of a convex optimization-based model predictive control (MPC) approach for providing guidance for ADR missions. Generally, while convex optimization can obtain the optimal solution in polynomial time, it relies on the convexification of nonconvex dynamics and constraints, leading to the need for successive convexification and inaccurate solutions. Here, the convex optimization scheme is improved by using the Generalized Equinoctial Orbital Elements (GEqOE) as they provide a near-linear-therefore, convex- representation of dynamics under $J_2$ perturbations. A highly accurate reference trajectory obtained through the Preliminary Mission Design Tool (PMDT) is also utilized to enhance the accuracy of the convex optimization. The convergence criteria are set using the proximity quotient of the Q-law, calculated for segments of the trajectory. Finally, the accuracy of the convex solution is measured with respect to a high-fidelity dynamics model that takes thrust misalignments, mistrust events, and navigational errors into consideration. If significant divergence exists between the convex solution and the high-fidelity trajectory, the reference trajectory from the current position to the target debris is recalculated through the PMDT.


==> oldupleg.tex <==
\newpage
\subsection{Fuel optimal up leg with perfect thrust implementation}



Figures \ref{foptb1} and \ref{foptb2} illustrate the fuel optimal results obtained. $DC'$ was set to 0.4 to obtain these results. The initial reference is a trajectory of $\Delta v = $ 161.99 m/s and $TOF = 66.47 $ days. The results with low fidelity and high fidelity dynamics are shown in Table \ref{tR}.


\begin{table}[hbt!]
\begin{tabular}{ccccccc}
Spacecraft Propagation & $\Delta a$ (km) & $\Delta i$ (deg) & $\Delta \Omega$ (deg) & TOF (d) & $\Delta v$ (m/s) & $\Delta v'$ (m/s) \\ \hline 
Low Fidelity           & -0.106973               & -0.002245               & -0.000339                                   & 66.4726 & 175.7491                      & 0.302740                       \\
High Fidelity          & -0.267798               & 0.000808                & -0.001287                                   & 66.4726 & 200.1975                      & 0.233326            \\ \hline           
\end{tabular}
\caption{Fuel optimal up leg with perfect thrust implementation}
\label{tR}
\end{table}

\begin{figure}[hbt!]
  \centering
  \begin{subfigure}[b]{0.49\textwidth}
  \centering
    \includegraphics[width = \textwidth]{Figures/foptb1.png}
    \caption{The fuel optimal solution with the high and low fidelity spacecraft propagations}
    \label{foptb1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width = \textwidth]{Figures/foptb3.png}
    \caption{The evolution of $\Delta v'$, semi-major axis, inclination, and RAAN errors with respect to the reference trajectories over time}
    \label{foptb2}
  \end{subfigure}
  \caption{Results of the up leg fuel optimal perfect thrust implementation}
  \label{fig:main}
\end{figure}




% \begin{figure}[hbt!]
%     \centering
%     \includegraphics[width = 0.8\textwidth]{Figures/foptb1.png}
%     \caption{The fuel optimal solution with the high and low fidelity spacecraft propagations}
%     \label{foptb1}
% \end{figure}
% \begin{figure}[hbt!]
%     \centering
%     \includegraphics[width = 0.8\textwidth]{Figures/foptb3.png}
%     \caption{The evolution of $\Delta v'$, semi-major axis, inclination, and RAAN errors with respect to the reference trajectories over time}
%     \label{foptb2}
% \end{figure}

\newpage
\subsection{Fuel optimal up leg with realistic thrust implementation}

 In this section, in the forward propagation of the spacecraft, the errors $p_{misthrust} = 1\%, \bar{\delta_T} = 5\%$ and $\bar{\delta_\beta} = 5$ deg are implemented on the convex-optimized thrust. The $DC'$ was again set to 0.4, and three sets of results were obtained for each of the high and low-fidelity forward propagations. The averaged results are shown in Table \ref{tR2}. Figures \ref{foptc1} and \ref{foptc2} illustrates the results.
 %The recomputations are conducted with $\epsilon = 2$ m/s.

\begin{table}[hbt!]
\begin{tabular}{ccccccc}
Spacecraft Propagation & $\Delta a$ (km) & $\Delta i$ (deg) & $\Delta \Omega$ (deg) & TOF (d) & $\Delta v$ (m/s) & $\Delta v'$ (m/s) \\ \hline 
Low Fidelity           & -0.3206                 & -0.005042               & 0.0006124                                   & 66.4726 & 176.2724                      & 0.4544                         \\
High Fidelity          & -0.0470                 & 0.0017420               & 0.0018049                                   & 66.4726 & 199.5737                      & 0.5150             \\ \hline           
\end{tabular}
\caption{Fuel optimal results with thrust implementation with errors}
\label{tR2}
\end{table}


\begin{figure}[hbt!]
  \centering
  \begin{subfigure}[b]{0.49\textwidth}
  \centering
    \includegraphics[width = \textwidth]{Figures/foptc1.png}
    \caption{The fuel optimal solution with the high and low fidelity spacecraft propagations}
    \label{foptc1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width = \textwidth]{Figures/foptc3.png}
    \caption{The evolution of $\Delta v'$, semi-major axis, inclination, and RAAN errors with respect to the reference trajectories over time}
    \label{foptc2}
  \end{subfigure}
  \caption{Results of the up leg fuel optimal realistic thrust implementation}
  \label{fig:main}
\end{figure}




% \begin{figure}[hbt!]
%     \centering
%     \includegraphics[width = 0.8\textwidth]{Figures/foptc1.png}
%     \caption{The fuel optimal solution with the high and low fidelity spacecraft propagations}
%     \label{foptc1}
% \end{figure}
% \begin{figure}[hbt!]
%     \centering
%     \includegraphics[width = 0.8\textwidth]{Figures/foptc3.png}
%     \caption{The evolution of $\Delta v'$, semi-major axis, inclination, and RAAN errors with respect to the reference trajectories over time}
%     \label{foptc2}
% \end{figure}

